The physics of deep-interior convective shell boundaries in a massive pre-supernova star: Internal gravity wave mixing at the $N^2$ peak

The physics of convective boundary mixing involves concepts such as penetration and overshooting and has been mostly characterized for envelope and core convection. For the burning shells deep inside massive stars in their final stages, the convective boundary remains poorly understood. 1D stellar-evolution codes typically place a steep entropy gradient and the corresponding narrow \brunt{} ($N^2$) peak at a lower convective shell boundary. Based on high-resolution 3D hydrodynamic simulations of a $25 \rm{M_\odot}$ star 11 days before core collapse, we find that convection excites high-frequency internal gravity waves at the $N^2$ peak representing the C-shell convection bottom. These waves efficiently mix entropy and species and the $N^2$ peak erodes by ${\sim}40\%$ within hours, correspondingly reducing the entropy gradient. The wave-driven diffusion coefficient is $D\approx 5\text{--}6\times 10^{9} \rm{cm}^2 \rm{second}^{-1}$ at the $N^2$ peak in numerically converged simulations. Our simulations show that the dominant physics at this boundary is mixing due to internal gravity waves. Extrapolated with the time-dependent $D$ coefficient from the 3D simulations, the entropy step across the peak decreases by 40--85\% within half a day, thereby reducing the density, temperature and entropy gradients that set the accretion-rate drop a stalled supernova shock encounters. This physics is not included in present-day 1D models and enters the structural parameters that predict explodability. Flattening the gradients days before collapse favors an O--C shell merger, which could reshape pre-collapse nucleosynthesis. Without this physics 1D models carry too sharp gradients that introduce previously unaccounted systematic errors into the explodability surveys, yield tables and chemical-evolution studies built on them.

==> hydropaper-resources/macros/units.tex <==
% $Id: units.tex 385 2008-07-13 20:07:02Z efb $

%------------------------------------------------------------------------
% typesetting of units
%
% Note that this doesn't prevent linebreaking between symbol and unit.
% siunitx is required for standard unit typesetting (\unit, \qty, \num, etc.)
%------------------------------------------------------------------------
\RequirePackage{siunitx}

% basic unit typesetteing
\newcommand{\unitspace}{\ensuremath{\,}}
\newcommand{\usp}{\unitspace}
\newcommand{\numberspace}{\ensuremath{\;}}
\newcommand{\nsp}{\numberspace}
\newcommand{\unitstyle}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\hour}{\unitstyle{h}}

\newcommand{\power}[2]{\ensuremath{{#1}^{#2}}}
\newcommand{\natlog}[2]{\ensuremath{#1\times 10^{#2}}} % a*10^b   
\newcommand{\ee}[1]{\ensuremath{\times 10^{#1}}}

% prefixes
\newcommand{\nano}{\unitstyle{n}}
\newcommand{\milli}{\unitstyle{m}}
\newcommand{\centi}{\unitstyle{c}}
\newcommand{\kilo}{\unitstyle{k}}
\newcommand{\Mega}{\unitstyle{M}}
\newcommand{\Giga}{\unitstyle{G}}

% base units, mks
\newcommand{\meter}{\unitstyle{m}}
\newcommand{\kilogram}{\kilo\gram}
\newcommand{\second}{\unitstyle{s}}
\newcommand{\Kelvin}{\unitstyle{K}}
\newcommand{\K}{\Kelvin}  %degrees Kelvin

% base units, cgs
\newcommand{\cm}{\centi\meter}
\newcommand{\gram}{\unitstyle{g}}

% derived units
\newcommand{\grampercc}{\gram\usp\power{\cm}{-3}} %mass density
\newcommand{\grampersquarecm}{\gram\usp\power{\cm}{-2}} %column depth
\newcommand{\squarecmpergram}{\power{\cm}{2}\usp\power{\gram}{-1}} %opacity
\newcommand{\GramPerCc}{\grampercc}
\newcommand{\GramPerSc}{\grampersquarecm}
\newcommand{\columnunit}{\grampersquarecm}
\newcommand{\dyne}{\unitstyle{dyn}} %dyne
\newcommand{\erg}{\unitstyle{ergs}} %ergs
\newcommand{\ergs}{\erg}
\newcommand{\gauss}{\unitstyle{G}} %gauss
\newcommand{\ergspersecond}{\erg\unitspace\power{\second}{-1}}
\newcommand{\ergspergram}{\erg\unitspace\power{\gram}{-1}}
\newcommand{\ergspergs}{\erg\unitspace\power{\gram}{-1}\unitspace\power{\second}{-1}} %angular momentum
\newcommand{\ergssecond}{\erg\unitspace\second}
\newcommand{\cgsflux}{\erg\unitspace\power{\cm}{-2}\usp\power{\second}{-1}}

% Nuclear and atomic units
\newcommand{\amu}{\unitstyle{u}} %atomic mass unit
\newcommand{\angstrom}{\mbox{\AA}} %Angstrom
\newcommand{\fermi}{\unitstyle{fm}} %fermi
\newcommand{\eV}{\unitstyle{eV}}        %eV
\newcommand{\keV}{\kilo\eV} %Kev
\newcommand{\MeV}{\Mega\eV} %MeV
\newcommand{\pcc}{\power{\cm}{-3}} % per cubic-centimeter
\newcommand{\pmbarn}{\unitstyle{\power{mbarn}{-1}}} %per mbarn                          

% solar and astronomical units
\newcommand{\Msun}{\ensuremath{\unitstyle{M}_\odot}}
\newcommand{\Lsun}{\ensuremath{\unitstyle{L}_{\odot}}}
\newcommand{\Rsun}{\ensuremath{\unitstyle{R}_{\odot}}}
\newcommand{\Zsun}{\ensuremath{Z_{\odot}}}
\newcommand{\Myr}{\Mega\yr}
\newcommand{\Gyr}{\Giga\yr}
\newcommand{\parsec}{\unitstyle{pc}}
\newcommand{\kpc}{\kilo\parsec} %kiloparsec
\newcommand{\mJy}{\unitstyle{\mu Jy}} %micro Jansky
\newcommand{\Msunyr}{\Msun\,\power{\yr}{-1}}
\newcommand{\MJ}{\ensuremath{\mathrm{M_J}}}
\newcommand{\RJ}{\ensuremath{\mathrm{R_J}}}
\newcommand{\AU}{\unitstyle{AU}}

% misc. units
%\newcommand{\hour}{\unitstyle{h}}
\newcommand{\minute}{\unitstyle{min}} %minute
\newcommand{\yr}{\unitstyle{yr}}        %year
% note that Latex defines \day as a counter
% see http://latexref.xyz/_005cday-_0026-_005cmonth-_0026-_005cyear.html
% therefore we use here the plural form
\newcommand{\days}{\unitstyle{d}}        %day  
\newcommand{\km}{\kilo\meter}   %kilometers
\newcommand{\Mm}{\Mega\meter}   %megameters
\newcommand{\Hz}{\unitstyle{Hz}}        %Hertz
\newcommand{\ksec}{\kilo\second} %kilosecond
\newcommand{\kms}{\ensuremath{\mathrm{km}\,\second^{-1}}\xspace}
\newcommand{\vcrit}{{\varv_{\mathrm{crit}}}}
\newcommand{\vkep}{{\varv_{\mathrm{kep}}}}
\newcommand{\vsurf}{{\varv_{\mathrm{surf}}}}
\newcommand{\mol}{\unitstyle{mol}}% mole
\newcommand{\barn}{\unitstyle{b}} %barn
\newcommand{\Hp}{\ensuremath{\unitstyle{H_P}}}
\newcommand{\Hpzero}{\ensuremath{\unitstyle{H_{P0}}}}
\newcommand{\OP}{\ensuremath{\unitstyle{OP}}} % overproduction

% Legacy \unit command — commented out to avoid conflict with siunitx.
% Use \qty{value}{unit} (siunitx v3) or \SI{value}{unit} (siunitx v2) instead.
%\newcommand{\unit}[2]{\ensuremath{#1\numberspace\mathrm{#2}}}


==> hydropaper-resources/macros/vectors.tex <==
%=======================================================================
%
% vectors.tex---some basic vector operators
%
% Requires package bm.sty
%
%=======================================================================

\RequirePackage{bm}
%\RequirePackage{amssymb}
%\RequirePackage{amsbsy}
\newcommand{\bvec}[1]{\ensuremath{\boldsymbol{#1}}} %boldface vector style
\newcommand{\grad}{\bvec{\nabla}} %gradient
\newcommand{\divr}{\nabla \cdot} %divergence
\newcommand{\curl}{\bvec{\nabla \times}} %curl
\newcommand{\lap}{\ensuremath{\nabla^2}} %Laplacian
\newcommand{\btens}[1]{\ensuremath{\boldsymbol{\mathsf{#1}}}}
\newcommand{\vcross}{\bvec{\times}}
\newcommand{\vdot}{\bvec{\cdot}}
\newcommand{\vort}{\ensuremath{|\curl u|}}
\newcommand{\vortsq}{\ensuremath{\vort^2}}
% end vectors.tex

